HIKE, High Intensity Kaon Experiments at the CERN SPS

A timely and long-term programme of kaon decay measurements at a new level of precision is presented, leveraging the capabilities of the CERN Super Proton Synchrotron (SPS). The proposed programme is firmly anchored on the experience built up studying kaon decays at the SPS over the past four decades, and includes rare processes, CP violation, dark sectors, symmetry tests and other tests of the Standard Model. The experimental programme is based on a staged approach involving experiments with charged and neutral kaon beams, as well as operation in beam-dump mode. The various phases will rely on a common infrastructure and set of detectors.

==> TimescaleCost.tex <==
\section{Timescale and cost estimate}

==> beam.tex <==
\section{High-intensity beams (Bernhard, Doble, Holzer, Gatignon)}

As the acronym HIKE suggests, the beam line must provide significantly higher beam intensities than those that are now delivered to the NA62 experiment, in the order of 4 to 6 times of that currently provided, which would correspond to between 1.2 and $2 \times 10^{13}$ protons on target per SPS extraction. Here, we assume that a typical running year has 200 days with 3000 spills each, including an SPS uptime of about 80~\%, and a flat top length of 4.8~seconds.

The proposed HIKE program includes both a charged beam ($K^{+}$) phase as well as a neutral beam ($K_{L}$) phase, respectively. For both parts of the program, protons at much higher intensity have to be transported via the P42 beam https://www.overleaf.com/project/62c2cbe919d8544710b9c6adline from the T4 target to the kaon production target. Conceptually, the $K^+$ beam is proposed to be the same as the present beam line, but consolidation and upgrades are needed to handle the higher beam intensities. Improved beam instrumentation will keep the beam losses better under control. A more precise calibration of the primary beam intensity measurements by the secondary emission monitors at T4 and T10 is important for beam optimisation, and also for normalisation purposes in dump mode. Efforts in this respect have already been started by the BI and EA groups at CERN.
The neutral beam line is an entirely new design and requires minor local modifications to the last section of the P42 line.

\subsection{Beam delivery to the kaon production target}

The P42 beam line started operation in 1980 and hardly has been modified since then~\cite[Chapter 5]{Banerjee:2774716}. Most of the equipment dates from then and is showing strong effects of ageing. Many issues and suggestions for mitigation have been described in the report from the PBC Conventional Beams working group~\cite{Gatignon:2650989}, which has recently been updated. The first phase of a vast consolidation program for the CERN North Area, titled NA-CONS, has recently been approved and funded, and the second phase has been prepared~\cite{Kadi:2018, Kadi:2019, Kadi:2021}. This will allow to bring the equipment and beam infrastructure back into a reliable state. Some upgrades are required to cope with the up to 6 times higher beam intensity, including operational requirements from the rest of the North Area complex and with stricter safety and radiation protection requirements compared to the original installation. Many studies have been performed by the SPS Losses and Activation working group (SLAWG)~\cite{Balhan:2668989, Fraser:ipac17-mopik045, Fraser:ipac19-wepmp031}, the Physics Beyond Collider (PBC) Proton Delivery working group~\cite{KoukoviniPlatia:2675225}, the PBC Conventional Beams working group~\cite{Gatignon:2650989}, and more recently, by the PBC ECN3 beam delivery task force~\cite{Brugger:2022}, focusing on the possibility to extract and deliver such high intensities towards TCC8 and ECN3.

The present beam optics of the P42 beam is shown in Fig.~\ref{fig:P42optics}. In order to reduce the attenuation of the primary beam in the T4 target, several options are considered. One is to increase the vertical beam size so that most of the beam by-passes the target without interacting. Another option is to run dedicated cycles for ECN3 in which the beam is bumped to pass above or below the target plate. This option could allow in principle even higher intensities than $2 \times 10^{13}$ ppp on the T10 target.
At present, the beam is provided in spills of 4.8~seconds, typically twice per super-cycle of about 40 to 45~seconds during day time, and two equally-spaced spills during 33.6~seconds during nights. One spill every 14.4~seconds is technically possible, as well. In recent years, on average 3000~spills per day are delivered, including the typical availability of SPS beams of about 80\%. The figure of merit is the time on flat top per year, which is proportional to the duty cycle and the running time. It is also important that the beam intensity is delivered as uniformly as possible. At the time of the NA62 proposal one assumed an effective spill of 3.3~seconds, but thanks to recent improvements we anticipate that it can be significantly better, ideally better than 4~seconds for a 4.8~second spill. The spill length can be modified to some extent, but it is important to maintain the duty cycle as well as the instantaneous intensity, respecting both the RMS power limitation of the SPS and transfer lines as well as the maximum intensity that the SPS is able to accelerate. The latter implies that the intensity per spill shall be kept proportional to the spill length.

\begin{figure}[htp]
\centering
\includegraphics[width=\textwidth]{figs/P42optics.png}
\caption{The beam optics for the P42 primary beam line, delivering protons from the T4 production target to the T10 Kaon production target. The red line depicts the local values of the R12 (horizontal) and R34 (vertical) beam transport matrix terms. The dotted blue line shows the local dispersion terms R16 (horizontal) and R36 (vertical).}
\label{fig:P42optics}
\end{figure}

Studies by the SY-STI group in the PBC context suggest that the P4 TAXs are already now running close to the maximum intensity allowed~\cite{Gatignon:2650989}. An upgrade is being studied at the technical level in the framework of the ECN3 task force. It will probably require a different choice of material in the TAX blocks and cooling closer to the beam impact point.
The present interlocks, P0-Survey and Dump Control, protect both the beam line equipment and the NA62 experiment against wrong magnet currents, T10 target and K12 TAX cooling problems and closed vacuum vales in the K12 beam line. For the higher intensities in the future, this system must be sped up. This is planned within the NACONS program baseline, independent of the proposed high intensity upgrade for ECN3, profiting from a new generation of power converters. On the shorter time scale some improvements are already under consideration, compatible with the presented HIKE timeline.  
Many studies are on-going concerning radiation dose levels to equipment and on surface, which must remain under control also at the higher intensities. All these issues will be addressed in the forthcoming report from the ECN3 beam delivery task force.

For a $K_L \rightarrow \pi^{0}\nu\bar{\nu}$ experiment, the production angle of the kaon beam has to be increased to 8~mrad instead of the zero production angle used for the charged mode. This can be achieved by a minor modification of the P42 beam line, i.e. realigning the three last dipoles as documented in the Conventional Beams Working Group Report~\cite{Gatignon:2650989}, shown in Fig.~\ref{fig:prodangleklever}. 
The high-intensity proton beam will ultimately impinge on the kaon production target, followed by the TAX beam dumps. These will need to be upgraded to withstand the higher beam power. A new target design could be inspired by the concepts of the CNGS target, which survived similar intensities with a fast extraction. The target material might be changed from Beryllium to Carbon for better handling. However, also more dense target materials can be considered as an option outside of the present baseline, as they could be advantageous in particular for the neutral beam line. The new K12 TAX will probably be based on the concept that is developed for the P42 TAX. TAX holes will be defined to ensure compatibility with the charged beam as well as the neutral beam.

\begin{figure}[htp]
\centering
% trim={<left> <lower> <right> <upper>}
\includegraphics[width=\textwidth, trim={3cm 0.1cm 0 3cm},clip]{figs/prod_angle_klever.jpg}
\caption{Modifications of the T10 target steering dipoles for increasing the production angle to 8~mrad, as required for the KLEVER part of HIKE.}
\label{fig:prodangleklever}
\end{figure}

%%%%%%%%%%%%%%%%

\subsection{The charged beam line}

The charged beam line for HIKE will remain conceptually as it is now, with essentially the same beam properties apart from the beam intensity (Fig.~\ref{fig:K12optics}). Consolidation of some equipment is required in the framework of NACONS, such as the K12 machine protection system in synergy with the P42 interlock upgrade. The main upgrades concern the T10 production target and the K12 TAX, including the needed shielding. A pre-study was presented in the Conventional Beams Working Group report~\cite{Gatignon:2650989} and is being followed-up further in that same working group. 

\begin{figure}[htp]
  \centering
  \includegraphics[width=0.9\textwidth]{figs/K12_optics.jpg}
  \caption{The beam optics for the K12 beam line. The red line depicts the local values of the R12 (horizontal) and R34 (vertical) beam transport matrix terms. The dotted black line shows the local dispersion terms R16 (horizontal) and R36 (vertical).}
  \label{fig:K12optics}
\end{figure}

The K12 beam itself is a mixed beam, which contains about 6.5\% of kaons at 75~GeV/$c$. A study has been performed to evaluate if the beam can be enriched by RF separation. Unfortunately, RF separation requires a much longer beam line, which implies that more kaons decay before the fiducial volume. This decreases not only the kaon flux but also the initial kaon fraction in the beam before enrichment. It turns out that a RF-separated beam cannot fulfil the HIKE requirements, even with state-of-the-art RF systems.

%%%%%%%%%%%%%%%%
\subsection{The $K_{L}$ beam for an experiment with tracking}
We propose a second phase with a neutral beam, but a detector very similar to the charged experiment, thus including a tracking system.

For the KLEVER part of the HIKE proposal, a neutral beam line has been designed and presented in the Conventional Beams Working Group report~\cite{Gatignon:2650989}. The design is straightforwardly based on the experience with the $K_L$ beam lines for NA31 and NA48, following guidelines laid out in Ref.~\cite{Gatignon:2730780}. The design is schematically shown in Fig.~\ref{fig:klever_beam}.

\begin{figure}[htp]
\centering
\includegraphics[width=0.9\textwidth]{figs/klever_beam.pdf}
\caption{Neutral beam design for the KLEVER part of HIKE.}
\label{fig:klever_beam}
\end{figure}

The primary proton beam impinges on the T10 target with a downward vertical angle of 8~mrad. This production angle softens the $\Lambda$ spectrum, so that almost all decay before the start of the fiducial volume. The $K_{L}$ flux is also reduced and the spectrum is also softened, which in fact increases the fraction that decays in the fiducial volume. The target is immediately followed by a first collimator that stops hadrons outside the beam acceptance before they decay and produce muons. The non-interacting protons are swept further downward by a strong dipole magnet. The neutral beam is on a horizontal axis. The protons and charged secondaries are dumped in the TAX, which has apertures that allow the neutral beam to pass. A photon converter consisting of about 9~$X_0$ of high-Z material is positioned at the centre of the TAX between the two modules and reduces the flux of high-energy photons ($E > 5$~GeV) in the neutral beam by about two orders of magnitude. A thinner oriented crystal converter is an optional possibility under study. Shower products emerging from the TAX are swept horizontally by a dipole magnet. Three collimators define the beam acceptance in a clean way. The defining collimator is located at $1/3$ of the distance to the final collimator and defines the angular acceptance of the neutral beam to not more than $\pm$0.4~mrad, which is necessary to measure the transverse momentum $p_t$ of the $\pi^{0}$ to sufficient precision in order to reject background from $K_L \rightarrow \pi^{0}\pi^{0}$ decays. A cleaning collimator stops debris from scattering on the jaws of the cleaning collimator. It is roughly hallway in between the defining and the final collimator, which stops scattering products from the cleaning collimator. The defining and cleaning collimator are followed by strong sweeping magnets. The final collimator will be an active collimator and defines the start of the fiducial volume. There is a lot of space available to add more collimation stages, depending on future design iterations within the Conventional Beams working group.

The rates and spectra have been calculated and reported in the Conventional Beams Working Group report. \textit{Here follows what we get from Evgueni.}
This neutral beam line would start from the present T10 location. Its length is about 120 metres, which is 18 metres longer than the charged beam line. As the detectors cannot be moved downstream inside ECN3, this leads to a shortening of the fiducial volume. We are asking the Conventional Beams working group to study, as an option, the feasibility and performance of a modified beam line with a reduced length of 90 to 100 metres. This will be presented in the forthcoming proposal.

\subsection{The neutral beam line for a precise measurement of $K_{L} \rightarrow \pi^{0}\nu\bar{\nu}$}

After the initial neutral beam studies for the KLEVER phase of HIKE were completed, it was discovered that the background from $\Lambda\to\pi^0 n$ decays is more difficult to suppress than thought so far. Therefore, the amount of $\Lambda$ decays in the fiducial region has to be reduced further by several orders of magnitude, whilst preserving as much as possible the kaon flux. Lengthening the beam line by 150~m seems to be the best option. Several possibilities are under consideration. Moving the T10 target further upstream is one of them, but this may have complex radiation protection implications and might require the whole HIKE experiment to be installed on a slope, depending on the exact target location.
%% MM: My understanding was that if the extension starts at TDC85 the beam line can be level JB: (Hopefully) fixed, see above.
The more straightforward option is to prolong the ECN3 cavern by 150~m, implying civil engineering works. Simulations show that this brings the background from $\Lambda$ decays to an acceptable level. The technical details and costs of the different options are under discussion with the Civil Engineering group of CERN. 

\textit{Here we can insert the input from Matthew}

An extension of the ECN3 cavern implies that the detector will be installed 150~m downstream of the present NA62 location.

In case resources allow to advance the construction of the ECN3 extension, the $K_{L}$ experiment with tracking could possibly also be performed with the extended beam line and the detector in the new location.

% In a first phase of the $K_{L}$ program, a simplified neutral beam, however at reduced flux and performance, can be used in alternation with the charged beam program by minor changes to the charged beam line. In such a case, a neutral beam can be transported all the way to the end of the ECN3 hall. With respect to the current layout of the beam line, only the magnetic collimator has to be removed and replaced by a vacuum tube. The front-end achromat will be sapped to sweeping mode. The magnet settings at the end of the P42 line will be changed to provide a production angle of 2.4~mrad, in the same way as it was done for the operation of the NA48 experiment. The experiment is then essentially the charged detector, including tracking. 

% \begin{figure}[htp]
% \centering
% \includegraphics[width=0.9\textwidth]{figs/K12symmetricLayout.pdf}
% \vspace{-5mm}
% \caption{Initial design of a symmetric beam layout.}
% \label{fig:K12symmetric}
% \end{figure}

% The present NA62 beam line K12, and therefore initial HIKE layout, deflects the charged beam using a corrector magnet (TRIM5) before the start of the decay volume and then in the opposite direction using the spectrometer magnet MNP33. As a consequence, the small dead zones (holes) in the straw detectors are offset away from the straight beam axis. A neutral beam cannot be deflected and the dead zones would have to be on axis, hence all straw detectors would have to be moved horizontally. To mitigate this problem, a so-called symmetric beam layout option is under study. It requires the installation of a second MNP33-like spectrometer magnet. On a side note, one should mention that the present MNP33 magnet consumes a lot of power, as the design was not optimised for power consumption. With a new magnet design, the power consumption per magnet can be reduced significantly. In such a layout, the straw chambers also can keep their positions. All changes occur only from TRIM5 onward and the beam parameters are otherwise unchanged. A possible preliminary layout of this scheme is shown in Fig.~\ref{fig:K12symmetric}. %The symmetric layout could be installed after a first phase of the K+ experiments in HIKE, i.e. after LS4 at the earliest. 



% This includes beam instrumentation and calibration

% HIKE proposes to use the upgraded K12 beams from the SPS and the experimental hall ECN3, where NA62 is currently installed.

% The SPS provides 400~GeV/$c$ proton beams to the North Area experiments and test beam lines. A typical SPS North Area cycle (SFTPRO cycle) lasts 10.8 to 14.4 seconds with the slow extraction lasting for about 4.8~s. Beam septa intercept the extracted beams and split them into three separate branches. These, now separated beams, impinge on the T2, T4 and T6 primary target respectively with a pre-selected sharing of the number of protons on each target (POT). Summer 2022 saw a record beam intensity with more than $4\cdot10^{13}$ protons in the SFTPRO cycle of the SPS and a combined number of POT on the three targets approaching $3\cdot 10^{13}$. Two secondary beams are derived from the protons interacting in the T4 target, the H6 and H8 beams for the EHN1 hall. The protons which do not interact in the T4 target are guided through the approximately 823~m long P42 beam line onto the T10 target, where the K12 beam line originates.%
% \footnote{An alternative path for the protons is available via target T6 (along a beam line, P62, which, after the first approximately 130~m, joins and thereafter follows the same path as P42), on condition that the front-end (pion decay section) of the M2 muon beam from target T6 is set to a momentum of $-200$~GeV/$c$ for $+400$~GeV/$c$ in P62.}

% Secondary particles at momenta of 75~GeV/c, most copiously pions, protons and kaons, are selected and transported through the approximately 102~m long K12 beam line towards the experiment installed in the underground cavern EHN3.

% The nominal intensity for NA62 is $35\cdot10^{11}$ POT on T10 corresponding to $70\cdot10^{11}$ POT on T4, both numbers as measured with the beam instrumentation calibration of summer 2022.

% \begin{itemize}
% \item Four times 2022 intensity on T10 (charged Kaon beam)
% \item beam properties similar? same? as in 2022?
% \item EHN3 task force /  EABI Working Group / NACONS
% \item Additional beam instrumentation for the coming years
% \item Additional beam instrumentation for the high intensity upgrade (EHN3 task force)
% \item North Area Consolidation Project (NACONS)
% \item The projections for HIKE assume the same effective spill length as currently in NA62, which is approximately 4 seconds and about the same average number of SPS spills per day, which is in the order of 3000 spills per day averaged over all the days of the run (including Technical Stops, dedicated MDs etc.
% \item Base the chapter on the snowmass paper.  high Z target for $K_L$ only as one option (the other one being to keep the same low Z target for $K_L$ as we have for $K^+$).
% \item Measurement of beam intensity on the T10 target to 5--10\% required for the measurements in ``dump'' mode and for the neutral kaon measurements.
% \end{itemize}


==> electronics.tex <==
\section{Common electronics (Fantechi, Lichard, Zamkovsky)}

==> introduction.tex <==
\section{Introduction (Giuseppe and Cristina)}

Over 75~years, experimental studies of kaon decays have played a singular role in propelling the development of the Standard Model. As in other branches of flavour physics, the continuing experimental interest in the kaon sector derives from the possibility of conducting precision measurements, particularly of suppressed or rare processes, that may reveal the effects of new physics with mass-scale sensitivity exceeding that which can be explored directly, e.g., at the LHC or a next-generation hadron collider. Because of the relatively small number of kaon decay modes and the relatively simple final states, combined with the relative ease of producing intense kaon beams, kaon decay experiments are in many ways the quintessential intensity-frontier experiments.

Over the past four decades, the CERN North Area has been hosting a successful series of precision kaon decay experiments. Among the many results obtained by these experiments is the discovery of direct CP violation, widely quoted to be among the top 10 discoveries made at CERN. Continuation of high-intensity kaon experiments at CERN, including future upgrades (providing a unique probe into BSM physics complementary to the $B$-sector) has been identified as an essential scientific activity in the 2020 Update of the European Strategy for particle physics, and is strongly supported in the national roadmaps across Europe.

The High-Intensity-Kaon-Experiments (HIKE) project represents a broad, long-term programme at CERN after LS3, based in the North Area ECN3 experimental hall, covering all the main aspects of rare kaon decays and searches accessible via kaon physics, from ultra-rare kaon decays to precision measurements and searches for new phenomena. 
HIKE is intended to continue the very successful tradition of kaon experiments at CERN in ECN3, where currently operating NA62 is the latest of the experiments. HIKE will profit from a beam intensity higher by a factor between four and six than that of NA62, and cutting-edge detector technologies to perform precision measurements and New Physics (NP) searches.
This will allow HIKE to play a pivotal role in the quest for NP at the sensitivity required by the present experimental limits and theoretical models, in a wide range of possible masses and interaction couplings.

The programme will consist of multiple phases, initially with charged and then neutral kaon beams, and periods in beam dump mode. The long decay volume and detector characteristics needed for kaon physics make HIKE suitable to search for new feebly-interacting, long-lived particles, providing unique sensitivity to forward processes. The detector is challenging but at least one technological solution exists for each detector, thanks also to the synergy with HL-LHC. The various phases allow for insertion, repositioning or removal of specific detector elements depending on the physics requirements, while the overall setup is maintained broadly the same.
%HIKE is expected to be divided into three phases:
%\begin{enumerate}
%    \item {\bf Charged kaon mode}: $K^+$ physics will be scrutinized with the highest precision expanding and improving the physics program of the NA62 experiment presently running in ECN3. New detectors will replace those of NA62 with the goal to improve the performance and sustain the higher rates. For example, HIKE will approach the ultimate theory uncertainty in the measurement of $Br(K^+ \rightarrow \pi^+ \nu \nu )$. A dump beam configuration to study feebly interacting particles can also be realised without detector modification, and a factor 10 improvement in sensitivity is expected with respect to what NA62 can achieve by LS3. The general sharing of the beam time between kaon and dump mode is discussed in section~\ref{sec:xxx}. 
%    \item {\bf Neutral kaon mode with tracking}: $K_L$ physics will be addressed, in particular $K_L$ decays with charged particles in the final state. This mode will require minimal modifications of the detector layout with respect to the charged mode. The dump beam configuration can happen also in this mode, with an appropriate time sharing with the kaon mode. The setup with tracking devices will also represent an opportunity to study in detail the composition of the neutral beam before moving to the third phase.
%    \item {\bf Neutral kaon mode without tracking (KLEVER)}: the experimental apparatus will be modified to address specifically the $K_L\rightarrow\pi^0\nu\bar{\nu}$ decay.
%\end{enumerate}
%The charged kaon mode will run between LS3 and LS4; the neutral kaon mode between LS4 and LS5; the P0NN mode after LS5.

